Reflections on Termination of Linear Loops

This paper shows how techniques for linear dynamical systems can be used to reason about the behavior of general loops. We present two main results. First, we show that every loop that can be expressed as a transition formula in linear integer arithmetic has a best model as a deterministic affine transition system. Second, we show that for any linear dynamical system $f$ with integer eigenvalues and any integer arithmetic formula $G$, there is a linear integer arithmetic formula that holds exactly for the states of $f$ for which $G$ is eventually invariant. Combining the two, we develop a monotone conditional termination analysis for general loops.

==> pratenddefaultcategory.tex <==

\prAtEndRestateiii*
\label{proofsection:prAtEndiii}\begin{proof}[\autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Define $A$ to be the transition system whose transition relation is the affine hull of the transition relation of $F$. Clearly, the identity function is a simulation from $F$ to $A$ since $R_F \subseteq R_A = \aff (F)$. Suppose that $U$ is an affine transition system and that $s : F \rightarrow U$ is a linear simulation. Then $s$ is also a linear simulation from $A$ to $U$, since $s^{-1}[R_U]$ is affine and contains $R_F$ (and therefore contains $\aff (F)$).\end{proof}
\prAtEndRestatevi*
\label{proofsection:prAtEndvi}\begin{proof}[\autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}By Lemma~\ref {lem:dual-space-simulation} it is sufficient to show that for any $f \in S_U^\star $, we have $f \circ s \in E_{\mathbb {Q}}(T)$. Suppose that $U$ has dimension $n$, and $\dom ^\omega (U)$ has dimension $m$. Since the set of functionals $f$ satisfying $f \circ s \in E_{\mathbb {Q}}(T)$ is linear, it is sufficient to construct a basis $f_1,\dots ,f_n$ for $S_U^\star $ and show that $f_i \circ s \in E_{\mathbb {Q}}(T)$ for each $i$. \par By the spectral theorem \cite [Ch. 6, Theorem 7]{Lax2007} and the assumption that $U$ has all rational spectrum, there is a basis for $\dom ^\omega (U)^\star $ consisting functionals $h_1,\dots ,h_m$ that for each $i$ there is some $\lambda _i \in \mathbb {Q}$ and $r_i \geq 1$ such that $h_i \circ (U|_\omega - \underline {\lambda _i})^{r_i} = 0$. For each $i$, let $f_i \in S_U^\star $ be an (arbitrary) extension of $h_i$ to $S_U$. Let $f_{m+1},\dots ,f_n \in S_U^\star $ be a basis for the space of functionals that vanish on $\dom ^\omega (U)$. Claim that $f_1,\dots ,f_n$ is linearly independent (and is therefore a basis for $S_U'$). Suppose that $a_1f_1 + \dots + a_nf_n = 0$; we must show $a_i$ = 0 for each $i$. For all $x \in \dom ^\omega (U)$ we must have \begin {align*} 0 &= (a_1f_1 + \dots + a_nf_n)(x) & \text {Assumption}\\ &= (a_1f_1 + \dots + a_mf_m)(x) & f_{m+1},\dots ,f_n \text { vanish on } \dom ^\omega (U)\\ &= (a_1h_m + \dots + a_mh_m)(x) & h_i \text { and } f_i \text { coincide on } \dom ^\omega (U) \end {align*} and thus $a_1 = \dots = a_m = 0$, since $h_1,\dots ,h_m$ are linearly independent. Since $a_{m+1}f_{m+1} + \dots + a_nf_n = 0$ and $f_{m+1}, \dots , f_n$ are linearly independent, we must have $a_{m+1} = \dots = a_n = 0$. \par Since $s : T \rightarrow U$ is a simulation, $s$ must map elements of $\dom ^\omega (T)$ to elements of $\dom ^\omega (U)$; we use $s|_\omega : \dom ^\omega (T) \rightarrow \dom ^\omega (U)$ to denote the restriction of $s$ to $\dom ^\omega (T)$. We have that $s|_\omega $ is a simulation from $T|_\omega $ to $U|_\omega $, which can be expressed by the equation $s|_\omega \circ T|_\omega = U|_\omega \circ s|_\omega $. From the construction of the basis $f_1,\dots ,f_n$, we have that $f_i \circ (U|_\omega - \underline {\lambda _i})^{r_i} = 0$ (for $i > m$, since $f_i$ vanishes on $\dom ^\omega (U)$ we may take $\lambda _i \defeq 0$ and $r_i \defeq 1$). Pre-composing with $s|_\omega $, we have $f_i \circ (U|_\omega - \underline {\lambda _i})^{r_i} \circ s|_\omega = 0$, and by induction on $r_i$, we have $f_i \circ s|_\omega \circ (T|_\omega - \underline {\lambda _i})^{r_i} = f_i \circ (U|_\omega - \underline {\lambda _i})^{r_i} \circ s|_\omega = 0$. We conclude that $f_i \circ s \circ (T|_\omega - \underline {\lambda _i})^{r_i} = 0$ and thus $f_i \circ s \in E_{\mathbb {Q}}(T)$.\end{proof}
\prAtEndRestatevii*
\label{proofsection:prAtEndvii}\begin{proof}[\autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Let $T$ be a $\DLTS {}$. Clearly, if Algorithm~\ref {alg:rational-spec-abstraction} terminates, then it returns a $\QDLTS {}$ abstraction of $T$. Since each iteration of the loop decreases the dimension the state space $S_U$, the algorithm must terminate. It remains to show that the abstraction is a reflection. \par Suppose that there exists a linear simulation $v$ from $T$ to an arbitrary $\QDLTS {}$ $V$. We show the loop maintains the invariant that there is a unique simulation $\overline {v} : U \rightarrow V$ such that $v = \overline {v} \circ s$. The invariant trivially holds when entering the loop. To show that it is maintained by the loop, we suppose that there exists a unique simulation $\overline {v} : U \rightarrow V$ such that $v = \overline {v} \circ s$, and show that there exists a unique simulation $\overline {v}' : U' \rightarrow V$ such that $v = \overline {v}' \circ d \circ q \circ s$, where $\tuple {Q,q} = \alpha _{E_\mathbb {Q}(U)}(U)$, and $\tuple {U',d} = \alpha _{\Det (Q)}(Q)$. \par Since $\overline {v}$ is a simulation from $U$ to $V$, by Lemma~\ref {lem:LTS-factor}, there exists a unique simulation $\overline {q}$ from $Q$ to $V$ such that $\overline {v} = \overline {q} \circ q$. Since $V$ is deterministic and $\tuple {U',d}$ is a deterministic reflection of $Q$, there exists a unique simulation $\overline {v}'$ from $U'$ to $V$ such that $\overline {q} = \overline {v}' \circ d$. We may then verify the desired result: \begin {align*} \overline {v}' \circ d \circ q \circ s &= \overline {q} \circ q \circ s = \overline {v} \circ s \end {align*} \par Finally, observe that $d \circ q \circ s$ is the composition of surjective maps and therefore surjective. It follows that $\overline {v}'$ is the \textit {unique} solution to the above equation.\end{proof}
\prAtEndRestateix*
\label{proofsection:prAtEndix}\begin{proof}[\autoref{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Define $t \defeq h \circ s$; observe that $t$ is a simulation from $F$ to $T$. \par By the spectral theorem, there is a basis $\vec {b}_1,\dots ,\vec {b}_n$ for $\dom ^\omega (T)$ such that for each $i$ there is some $\lambda _i \in \mathbb {Q}$ and some $r_i \in \mathbb {N}^{\geq 1}$ such that $(T|_\omega - \underline {\lambda _i})^{r_i}(\vec {b}_i) = 0$. We now argue that without loss of generality, we can further suppose that for all $v \in \dom ^\omega (F)$ such that $t(v) \in \dom ^\omega (T)$, there exist \textit {integers} $a_1,\dots ,a_n$ such that $t(v) = a_1\vec {b}_1 + \dots + a_n\vec {b}_n$. First, extend the basis $\vec {b}_1,\dots ,\vec {b}_n$ to a basis $\vec {b}_1,\dots ,\vec {b}_m$ for the whole space $S_T$. Let $\set {v_x}_{x \in X}$ denote the standard basis for $S_F = X \rightarrow \mathbb {Q}$, where where $v_x$ maps $x$ to 1 and all variables other than $x$ to $0$. Since $\vec {b}_1,\dots ,\vec {b}_m$ are rational vectors, there exist rationals $z_1,\dots ,z_m$ such that for each $v_j$, $t(v_j)$ is an integral linear combination of $z_1\vec {b}_1,\dots ,z_m\vec {b}_m$; $z_1\vec {b}_1,\dots ,z_m\vec {b}_n$ is a basis for $\dom ^\omega (T)$ with the desired property. To verify that for each $v \in \dom ^\omega (F)$, $t(v)$ is an integral combination of $z_1\vec {b}_1,\dots ,z_m\vec {b}_m$, observe that since $v \in \dom ^\omega (F)$, $v$ is an integral valuation and so $v$ is an integral combination of $\set {v_x}_{x \in X}$, and therefore $t(v)$ is an integral combination of $\vec {b}_1,\dots ,\vec {b}_m$. Since $t(v) \in \dom ^\omega (T)$, the coefficients of $\vec {b}_{n+1},\dots ,\vec {b}_m$ are zero. \par Since for each $i$ we have $(T|_\omega - \underline {\lambda _i})^{r_i}(\vec {b}_i) = 0$, we have for any $k$ and any $i$ such that $\lambda _i \neq 0$, $T|_\omega ^k(\vec {b}_i) = \lambda _i^k\vec {b}_i + \vec {v}$, where $\vec {v}$ satisfies $(T|_\omega - \underline {\lambda _i})^{r_i-1}(\vec {v}) = 0$ (i.e., $\vec {v}$ is a generalized eigenvector of lower rank). This can be shown by induction on $k$. The base case $k=0$ is trivial. For the inductive step, suppose $T|_\omega ^k(\vec {b}_i) = \lambda _i^k\vec {b}_i + \vec {v}$ with $(T|_\omega - \underline {\lambda _i})^{r_i-1}(\vec {v}) = 0$. Then \begin {align*} T|_\omega ^{k+1}(\vec {b}_i) & = T|_\omega (\lambda _i^k\vec {b}_i + \vec {v})\\ & = \lambda _i^k(T|_\omega (\vec {b}_i)) + T|_\omega (\vec {v})\\ &= \lambda _i^{k+1}\vec {b}_i + (T|_\omega (\vec {v}) + \lambda _i^{k}(T|_\omega (\vec {b}_i)) - \lambda _i^{k+1}\vec {b}_i)\\ &= \lambda _i^{k+1}\vec {b}_i + (T|_\omega (\vec {v}) + \lambda _i^{k}(T|_\omega - \underline {\lambda _i})(\vec {b}_i)) \end {align*} and we may verify \[ \begin {array}{ll} & (T|_\omega - \underline {\lambda _i})^{r_i-1}\left (T|_\omega (\vec {v}) + \lambda _i^{k}(T|_\omega - \underline {\lambda _i})(\vec {b}_i)\right )\\ =&T|_\omega ((T|_\omega - \underline {\lambda _i})^{r_i-1}(\vec {v})) + (T|_\omega - \underline {\lambda _i})^{r_i}(\vec {b}_i)\\ =& 0. \end {array} \] \par Suppose $v_0 \in \dom ^\omega (F)$. Then there exists an infinite trajectory \[ v_0 \rightarrow _F v_1 \rightarrow _F v_2 \rightarrow _F \dots \] and so there is an infinite trajectory \[ t(v_0) \rightarrow _T t(v_1) \rightarrow _T t(v_2) \rightarrow _T \dots \] and so $t(v_0) \in \dom ^\omega (T)$. We want to prove $t(v_0) \in \Int (T)$. \par Since for all $k$ we have $t(v_k) \in \dom ^\omega (T)$, there exists integers $c_{k,1},...,c_{k,n}$ such that $t(v_k) = c_{k,1}\vec {b}_1 + \dots + c_{k,n}\vec {b}_n$. Since $T|_\omega $ is the restriction of $T$ to $\dom ^\omega (T)$ and $T|_\omega $ is linear, we have \[ t(v_k) = (T|_\omega )^k(t(v)) = c_{0,1}(T|_\omega )^k(\vec {b}_1) + \dots + c_{0,n}(T|_\omega )^k(\vec {b}_n) \] \par Suppose for a contradiction that there is some $i$ with $c_{0,i} \neq 0$ and $\lambda _i$ is not an integer. Without loss of generality, further suppose that $\vec {b}_i$ has the greatest rank $r_i$ among all such indices. We will show that $c_{k,i} = \lambda _i^kc_{0,i}$ for all $k$, which is a contradiction since each $c_{k,i}$ is an integer and $\lambda _i$ is not an integer. \par By the above, for each $\vec {b}_j$ we have $T|_\omega ^k(\vec {b}_j) = \lambda _j^k\vec {b}_j + \vec {v}_j$ for some $\vec {v}_j$ satisfying $(T|_\omega - \underline {\lambda _j})^{r_i-1}(\vec {v}_j) = 0$, and we have \[ t(v_k) = (T|_\omega )^k(t(v)) = c_{0,1}(\lambda _1^k\vec {b}_1 + \vec {v}_1) + \dots + c_{0,n}(\lambda _n^k\vec {b}_n + \vec {v}_n) \] Since $r_i$ is maximal, every $\vec {v}_j$ is orthogonal to $\vec {b}_i$ (w.r.t. the basis $\vec {b}_1,\dots ,\vec {b}_n$), and so $c_{k,i}$ is simply $\lambda _i^kc_{0,i}$. \par \par \end{proof}


==> pratendhomogenization.tex <==

\prAtEndRestateviii*
\label{proofsection:prAtEndviii}\begin{proof}[\autoref{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Let $T$ be a deterministic affine transition system. If $R_T$ is empty, then it is a $\QDATS {}$ and we are done. Suppose $R_T$ is non-empty. By Lemma~\ref {thm:best-qdlts}, $\Hom (T)$ has a $\QDLTS {}$-reflection, say $\tuple {\hat {T},s}$. The intuition behind the argument is that we may ``dehomogenize'' $\hat {T}$ and $s$ to obtain a $\QDATS {}$-reflection $\tuple {Z,z}$ of $T$. \par In the following, for any product space $A \times B$, we use $\pi _1$ and $\pi _2$ to denote the first and second projection ($\pi _1(a,b) \defeq a$, $\pi _2(a,b) \defeq b$). Let $K$ be the linear transition system where $S_K = \mathbb {Q}$ and $R_K = \set { \tuple {s,s} : s \in \mathbb {Q} }$; intuitively $K$ captures the dynamics of the constant dimension introduced by the homogenization process. Clearly $\sim {\pi _2}{\Hom (T)}{K}$ is a simulation, and $K$ has rational spectrum. Since $\tuple {\hat {T},s}$ is a $\QDLTS {}$-reflection of $\Hom (T)$, there is a unique simulation $\sim {\overline {\pi _2}}{\hat {T}}{K}$ such that $\overline {\pi _2} \circ s = \pi _2$. Define $Z$ to be the affine transition system where \begin {align*} S_Z &= \{ x \in S_{\hat {T}} : \overline {\pi _2}(x) = 0 \}\\ R_Z &= \{ \tuple {x,x'} : \tuple {x + s(0,1), x' + s(0,1)} \in R_{\hat {T}} \} \end {align*} Observe that for any $x \in S_T$, we have $\overline {\pi _2}(s(x,0)) = \pi _2(x,0) = 0$, and so the function $z$ defined by $z(x) \defeq s(x,0)$ maps $S_T$ to $S_Z$. In fact, $z$ is a simulation from $T$ to $Z$: \begin {align*} \tr {T}{x}{x'} &\Rightarrow \tr {\Hom (T)}{\tuple {x,1}}{\tuple {x',1}} & \text {Def'n of $\Hom $}\\ &\Rightarrow \tr {\hat {T}}{s(x,1)}{s(x',1)} & \text {$s$ is a simulation}\\ &\Rightarrow \tr {\hat {T}}{(s(x,0)+s(0,1))}{(s(x',0)+s(0,1))} & \text {Linearity}\\ &\Rightarrow \tr {Z}{s(x,0)}{s(x',0)} & \text {Def'n of $R_Z$}\\ &\Rightarrow \tr {Z}{z(x)}{z(x')} & \text {Def'n of $z$} \end {align*} \par Next we show that $\Hom (Z)$ is isomorphic to $\hat {T}$, and therefore has rational spectrum. Define a bijective linear map $e : S_{\Hom (Z)} \rightarrow S_{\hat {T}}$ by $e(x,c) \defeq x + cs(0,1)$. We now show that $\tr {\Hom (Z)}{(x,c)}{(x',c)} \iff \tr {\hat {T}}{e(x,c)}{e(x',c)}$. Let $x_0,x_0'$ be such that $\tr {Z}{x_0}{x_0'}$. Unfolding the definitions of $\Hom (Z)$ and $Z$, we have {\footnotesize \begin {align} \tr {\Hom (Z)}{(x,c)}{(x',c)} &\iff \tr {Z}{(x + (1-c)x_0)}{(x' + (1-c)x_0')}\\ &\iff \tr {\hat {T}}{(x + (1-c)x_0 + s(0,1))}{(x' + (1-c)x_0' + s(0,1))} \label {eq:tr1} \end {align}} Since by assumption $\tr {Z}{x_0}{x_0'}$, we have \begin {equation} \label {eq:tr2} \tr {{\hat {T}}}{(x_0 + s(0,1))}{(x_0' + s(0,1))}\ . \end {equation} Since $R_{\hat {T}}$ is closed under linear combinations, we may add the transition in Eq.~(\ref {eq:tr1}) to the transition Eq.~(\ref {eq:tr2}) scaled by a factor of $(c-1)$ to see that \[ \tr {\Hom (Z)}{(x,c)}{(x',c)} \iff \tr {\hat {T}}{x + cs(0,1)}{x'+cs(0,1)} \iff \tr {\hat {T}}{e(x,c)}{e(x',c)}\ . \] \par Finally, we show that $\tuple {Z,z}$ is a $\QDATS {}$-reflection of $T$. Suppose that $Y \in \QDATS {}$ and $\sim {y}{T}{Y}$ is a simulation. Then we have a simulation $\sim {\Hom (y)}{\Hom (T)}{\Hom (Y)}$, and since $\tuple {\hat {T},s}$ is a $\QDLTS $-reflection of $\Hom (T)$ there is a unique simulation $\sim {\overline {\Hom (y)}}{\hat {T}}{\Hom (Y)}$ such that $\overline {\Hom (y)} \circ s = \Hom (y)$. Define a function $\overline {y} : S_Z \rightarrow S_Y$ by $\overline {y} \defeq \pi _1 \circ \overline {\Hom (y)}$. We now show that $y = \overline {y} \circ z$ and that $\overline {y}$ is a simulation from $Z$ to $Y$ (uniqueness follows from the fact that $z$ is surjective). \par First, we show that $y = \overline {y} \circ z$. Observe that for any $x \in S_T$, we have \begin {align*} \overline {y}(z(x)) & = \pi _1(\overline {\Hom (y)}(s(x))) & \text {Def'n of $\overline {y}$ and $z$}\\ &= \pi _1(\Hom (y)(x,0)) & \Hom (y) = \overline {\Hom (y)} \circ s\\ &= \pi _1(y(x),0) & \text {Def'n of $\Hom (y)$}\\ &= y(x) \end {align*} \par Second, we show that $\overline {y}$ is a simulation from $Z$ to $Y$. Claim that for any $x \in S_Z$, we have $\overline {\Hom (y)}(x + s(0,1)) = (\overline {y}(x),1)$. The fact that $\overline {y}$ is a simulation follows: \begin {align*} \tr {Z}{x}{x'}& \Rightarrow \tr {\hat {T}}{(x + s(0,1))}{(x' + s(0,1))} & \text {Def'n of $Z$}\\ &\Rightarrow \tr {\Hom (Y)}{\overline {\Hom (y)}(x + s(0,1))}{\overline {\Hom (y)}(x' + s(0,1))} & \text {$\overline {\Hom (y)}$ is a simulation}\\ &\Rightarrow \tr {\Hom (Y)}{(\overline {y}(x), 1)}{(\overline {y}(x'),1)} & \text {Claim}\\ &\Rightarrow \tr {Y}{\overline {y}(x)}{\overline {y}(x')} & \text {Def'n of $\Hom (Y)$} \end {align*} \par It remains to prove the claim. Observe that \begin {align*} \overline {\Hom (y)}(x + s(0,1)) &= \overline {\Hom (y)}(x) + \overline {\Hom (y)}(s(0,1)) & \text {Linearity}\\ &=\overline {\Hom (y)}(x) + \Hom (y)(0,1) & \Hom (y) = \overline {\Hom (y)} \circ s\\ &=\overline {\Hom (y)}(x) + (y(0),1) & \text {Def'n of $\Hom (y)$}\\ &=\overline {\Hom (y)}(x) + (0,1) & \text {Linearity}\\ &=(\pi _1(\overline {\Hom (y)}(x)), \pi _2(\overline {\Hom (y)}(x)) + 1)\\ &=(\overline {y}(x), \pi _2(\overline {\Hom (y)}(x)) + 1) & \text {Def'n of $\overline {y}$} \end {align*} so it is sufficient to show that $\pi _2(\overline {\Hom (y)}(x)) = 0$. Since $s$ is surjective, there is some $\tuple {a,b} \in S_{\Hom (T)} = S_T \times \mathbb {Q}$ with $s(a,b) = x$. Finally, we may verify \begin {align*} \pi _2(\overline {\Hom (y)}(x)) &= \pi _2(\overline {\Hom (y)}(s(a,b))) & \text {Def'n of $a,b$}\\ &= \pi _2(\Hom (y)(a,b)) & \Hom (y) = \overline {\Hom (y)} \circ s \\ &= \pi _2(y(a),b) & \text {Def'n of $\Hom (y)$}\\ &= \pi _2(a,b)\\ &= \overline {\pi _2}(s(a,b)) & \pi _2 = \overline {\pi _2} \circ s\\ &= \overline {\pi _2}(x) & \text {Def'n of $a,b$} \end {align*} and since $x \in Z$ we have $\overline {\pi _2}(x) = 0$.\end{proof}


==> pratendmonotonicity.tex <==

\prAtEndRestatexi*
\label{proofsection:prAtEndxi}\begin{proof}[\autoref{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\tuple {A_1,m_1}$ and $\tuple {A_2,m_2}$ be $\QDATS {}$-reflections of $F_1$ and $F_2$, respectively. Let $\tuple {T,h_1} = \Homogenize (A_1)$ and $\tuple {U,h_2} = \Homogenize (A_2)$ be their homogenizations. Define $t \defeq h_1 \circ m_1$ and $u \defeq h_2 \circ m_2$ to be affine simulations $t : F_1 \rightarrow T$ and $u : F_2 \rightarrow U$. Since $F_1 \models F_2$ and $ \tuple {A_2, m_2}$ is a $\QDATS {}$-abstraction of $F_2$, it is also an abstraction of $F_1$. Since $ \tuple {A_1, m_1}$ is the $\QDATS {}$-reflection of $F_1$, there exists a simulation $\bar {m} : A_1 \rightarrow A_2$ such that $m_2 = \bar {m} \circ m_1$. Then $\overline {u} \defeq \Hom (\overline {m})$ is a simulation from $T$ to $U$ such that $u = \bar {u} \circ t$. \par We prove the contrapositive $\neg \mp (F_1) \models \neg \mp (F_2)$, which by Lemma~\ref {lem:semantics-of-char-sequences} is equivalent\footnote {The definition of $\mp $ is given in Algorithm~\ref {alg:end-to-end-mp}. For the case of $F_1$, we use the state formula $\exists \vec {x}, \vec {x}'. F_1(\vec {x}, \vec {x}') \land \vec {y} = t(\vec {x})$ as the LIA formula $G$ in Lemma~\ref {lem:semantics-of-char-sequences}. Similarly, we use $\exists \vec {x}, \vec {x}'. F_2(\vec {x}, \vec {x}') \land \vec {w} = u(\vec {x})$ as the LIA formula for $F_2$.} to showing that for all $v \in S_{F_1}$ such that $t(v) \in \mathrm {SAT}^\infty (T, \exists \vec {x}, \vec {x}'. F_1(\vec {x}, \vec {x}') \land \vec {y} = t(\vec {x}))$, we have $u(v) \in \mathrm {SAT}^\infty (U, \exists \vec {x}, \vec {x}'. F_2(\vec {x}, \vec {x}') \land \vec {w} = u(\vec {x}))$ \par Let $v \in S_{F_1}$ such that $t(v) \in \mathrm {SAT}^\infty (T, \exists \vec {x}, \vec {x}'. F_1(\vec {x}, \vec {x}') \land \vec {y} = t(\vec {x}))$. By the definition of $\mathrm {SAT}^\infty $, we know that there exists an infinite trajectory $\vec {y}_1, \vec {y}_2, \dots \in \Int (T)$ such that $t(v) \rightarrow _T \vec {y}_1 \rightarrow _T \vec {y}_2 \rightarrow _T \dots $ and a $K \in \mathbb {N}$ such that for all $k \geq K$, $\exists \vec {x}, \vec {x}'. F_1(\vec {x}, \vec {x}') \land \vec {y}_k = t(\vec {x})$ holds. Since $\bar {u} : T \rightarrow U$ is a simulation, there is a corresponding trajectory in $U$: $\bar {u}(t(\vec {x})) \rightarrow _U \vec {w}_1 = \bar {u}(\vec {y}_1) \rightarrow _U \vec {w}_2 = \bar {u}(\vec {y}_2) \rightarrow _U \dots $. \par Let $k \geq K$. Since $\exists \vec {x}, \vec {x}'. F_1(\vec {x}, \vec {x}') \land \vec {y}_k = t(\vec {x})$ holds and $F_1 \models F_2$, we must have $\exists \vec {x}, \vec {x}'. F_2(\vec {x}, \vec {x}') \land \vec {y}_k = t(\vec {x})$ and thus $\exists \vec {x}, \vec {x}'. F_2(\vec {x}, \vec {x}') \land \overline {u}(\vec {y}_k) = \overline {u}(t(\vec {x}))$. Since $\overline {u}(\vec {y}_k) = \vec {w}_k$ and $\overline {u}(t(\vec {x})) = u(\vec {x})$, and the above holds for all $k \geq K$, it follows that $u(\vec {x}) \in \mathrm {SAT}^\infty (U, \exists \vec {x}, \vec {x}'. F_2(\vec {x}, \vec {x}') \land \vec {w} = u(\vec {x}))$.\end{proof}

